Opacus: User-Friendly Differential Privacy Library in PyTorch

We introduce Opacus, a free, open-source PyTorch library for training deep learning models with differential privacy (hosted at opacus.ai). Opacus is designed for simplicity, flexibility, and speed. It provides a simple and user-friendly API, and enables machine learning practitioners to make a training pipeline private by adding as little as two lines to their code. It supports a wide variety of layers, including multi-head attention, convolution, LSTM, GRU (and generic RNN), and embedding, right out of the box and provides the means for supporting other user-defined layers. Opacus computes batched per-sample gradients, providing higher efficiency compared to the traditional "micro batch" approach. In this paper we present Opacus, detail the principles that drove its implementation and unique features, and benchmark it against other frameworks for training models with differential privacy as well as standard PyTorch.

==> tables/embedding_memory.tex <==
\begin{table}
\footnotesize
\begin{center}
\begin{tabular}{l| r| r| r| r| r| r| r}
    \toprule
     \textbf{\texttt{num\_embeddings}} & \textbf{Batch size} & $(L/C) / b$  & $1 + L/C$ & $b/3$ & $b/2$ & \textbf{Factor (DP)} & \textbf{Difference}\\
    \midrule
    \multirow{6}{*}{1} & 1 & 0.3 & \textbf{1.3} & 0.3 & 0.5 & 1.2 & -11\%\\
     & 16 & 0.04 & \textbf{1.6} & 5.3 & 8 & 1.2 & -33\%\\
     & 32 & 0.02 & \textbf{1.6} & 10.7 & 16 & 1.2 & -36\%\\
     & 64 & 0.01 & \textbf{1.6} & 21.3 & 32 & 1.2 & -36\%\\
     & 128 & 0.005 & \textbf{1.6} & 42.7 & 64 & 1.2 & -36\%\\
     & 256 & 0.002 & \textbf{1.6} & 85.3 & 128 & 1.2 & -36\%\\
     & 512 & 0.001 & \textbf{1.6} & 171 & 256 & 1.2 & -36\%\\
    \midrule
    \multirow{6}{*}{10} & 1 & 2.7 & 3.7 & 0.3 & \textbf{0.5} & 1.6 & 68\%\\
     & 16 & 0.3 & \textbf{5.7} & 5.3 & 8 & 3.9 & -47\%\\
     & 32 & 0.2 & \textbf{6.0} & 10.7 & 16 & 4.4 & -38\%\\
     & 64 & 0.08 & \textbf{6.1} & 21.3 & 32 & 4.6 & -33\%\\
     & 128 & 0.04 & \textbf{6.1} & 42.7 & 64 & 4.7 & -30\%\\
     & 256 & 0.02 & \textbf{6.1} & 85.3 & 128 & 4.7 & -28\%\\
     & 512 & 0.01 & \textbf{6.1} & 171 & 256 & 4.8 & -28\%\\
    \midrule
    \multirow{6}{*}{100} & 1 & 26.3 & 27.3 & 0.3 & \textbf{0.5} & 1.7 & 70\%\\
     & 16 & 2.9 & 47.8 & 5.3 & \textbf{8} & 10.0 & 20\%\\
     & 32 & 1.5 & 50.6 & 10.7 & \textbf{16} & 17.0 & 6\%\\
     & 64 & 0.8 & \textbf{51.1} & 21.3 & 32 & 25.4 & -101\%\\
     & 128 & 0.4 & \textbf{51.1} & 42.7 & 64 & 31.2 & -64\%\\
     & 256 & 0.2 & \textbf{51.1} & 85.3 & 128 & 36.1 & -42\%\\
     & 512 & 0.1 & \textbf{51.1} & 171 & 256 & 38.6 & -32\%\\
    \midrule
    \multirow{6}{*}{1000} & 1 & 261 & 262 & 0.3 & \textbf{0.5} & 1.7 & 70\%\\
     & 16 & 29.0 & 464 & 5.3 & \textbf{8} & 11.5 & 30\%\\
     & 32 & 15.3 & 492 & 10.7 & \textbf{16} & 21.6 & 26\%\\
     & 64 & 7.7 & 497 & 21.3 & \textbf{32} & 41.0 & 22\%\\
     & 128 & 3.9 & 497 & 42.7 & \textbf{64} & 76.5 & 16\%\\
     & 256 & 1.9 & 497 & 85.3 & \textbf{128} & 137 & 6\%\\
     & 512 & 1.0 & 497 & \textbf{171} & 256 & 225 & 24\%\\
    \midrule
    \multirow{6}{*}{10000} & 1 & 2604 & 2605 & 0.3 & \textbf{0.5} & 1.7 & 71\%\\
     & 16 & 289 & 4631 & 5.3 & \textbf{8} & 11.8 & 32\%\\
     & 32 & 153 & 4903 & 10.7 & \textbf{16} & 22.3 & 28\%\\
     & 64 & 77.4 & 4952 & 21.3 & \textbf{32} & 43.4 & 26\%\\
     & 128 & 38.7 & 4952 & 42.7 & \textbf{64} & 85.2 & 25\%\\
     & 256 & 19.3 & 4952 & 85.3 & \textbf{128} & 167 & 24\%\\
     & 512 & 9.7 & 4952 & 171 & \textbf{256} & 326 & 21\%\\
    \midrule
    \multirow{6}{*}{20000} & 1 & 5208 & 5209 & 0.3 & \textbf{0.5} & 1.7 & 70\%\\
     & 16 & 579 & 9260 & 5.3 & \textbf{8} & 11.7 & 31\%\\
     & 32 & 306 & 9805 & 10.7 & \textbf{16} & 22.3 & 28\%\\
     & 64 & 155 & 9902 & 21.3 & \textbf{32} & 43.5 & 26\%\\
     & 128 & 77.4 & 9902 & 42.7 & \textbf{64} & 85.8 & 25\%\\
     & 256 & 38.7 & 9902 & 85.3 & \textbf{128} & 170 & 24\%\\
     & 512 & 19.3 & 9902 & 171 & \textbf{256} & 334 & 23\%\\
    \midrule
    \multirow{6}{*}{50000} & 1 & 13653 & 13654 & 0.3 & \textbf{0.5} & 1.7 & 70\%\\
     & 16 & 1517 & 24274 & 5.3 & \textbf{8} & 11.2 & 28\%\\
     & 32 & 803 & 25701 & 10.7 & \textbf{16} & 21.3 & 25\%\\
     & 64 & 406 & 25956 & 21.3 & \textbf{32} & 41.6 & 23\%\\
     & 128 & 203 & 25956 & 42.7 & \textbf{64} & 82.2 & 22\%\\
     & 256 & 101 & 25956 & 85.3 & \textbf{128} & 163 & 22\%\\
     & 512 & 50.7 & 25956 & 171 & \textbf{256} & 323 & 21\%\\
     \bottomrule
\end{tabular}
\end{center}
\caption{Comparison of measured and predicted (according to \cref{eq:memory}) memory increase factor from adding DP for various \texttt{num\_embeddings} and batch sizes $b$. $C$ is calculated as the size of the input and 2$\times$ the size of the labels (to account for model outputs) divided by $b$. Excluding when $b = 1$, formula $1 + L/C$ overestimates the memory increase factor while $b/3$ and $b/2$ underestimate it. }
\label{tab:embedding_memory}
\end{table}

==> tables/runtimes_forward_only.tex <==
\begin{table}
\begin{center}
\vspace{-0.4in}
\begin{tabular}{|l| r| r| r| r| r| r|} 
    \hline
     \textbf{Layer} & \textbf{Batch size} & \texttt{nn.module} & \texttt{DPModule} & \texttt{GSM(module)} & \textbf{Factor (DP)}\\
     \hline
        Conv & 16 & 1.80 & n/a & 1.81 & 1.00\\
        Conv & 32 & 2.84 & n/a & 2.84 & 1.00\\
        Conv & 64 & 4.91 & n/a & 4.90 & 1.00\\
        Conv & 128 & 9.02 & n/a & 9.03 & 1.00\\
        Conv & 256 & 17.51 & n/a & 17.54 & 1.00\\
        Conv & 512 & 35.22 & n/a & 35.30 & 1.00\\
        \hline
        LayerNorm & 16 & 0.02 & n/a & 0.05 & 2.27\\
        LayerNorm & 32 & 0.02 & n/a & 0.05 & 2.25\\
        LayerNorm & 64 & 0.02 & n/a & 0.05 & 2.19\\
        LayerNorm & 128 & 0.02 & n/a & 0.05 & 2.21\\
        LayerNorm & 256 & 0.02 & n/a & 0.05 & 2.26\\
        LayerNorm & 512 & 0.02 & n/a & 0.05 & 2.20\\
        \hline
        InstanceNorm & 16 & 0.06 & n/a & 0.09 & 1.62\\
        InstanceNorm & 32 & 0.07 & n/a & 0.10 & 1.28\\
        InstanceNorm & 64 & 0.13 & n/a & 0.13 & 1.01\\
        InstanceNorm & 128 & 0.25 & n/a & 0.25 & 1.00\\
        InstanceNorm & 256 & 0.56 & n/a & 0.56 & 1.00\\
        InstanceNorm & 512 & 1.12 & n/a & 1.12 & 1.00\\
        \hline
        GroupNorm & 16 & 0.03 & n/a & 0.06 & 2.01\\
        GroupNorm & 32 & 0.03 & n/a & 0.06 & 2.00\\
        GroupNorm & 64 & 0.03 & n/a & 0.06 & 1.99\\
        GroupNorm & 128 & 0.03 & n/a & 0.06 & 2.02\\
        GroupNorm & 256 & 0.03 & n/a & 0.06 & 2.02\\
        GroupNorm & 512 & 0.03 & n/a & 0.06 & 1.97\\
        \hline
        Linear & 16 & 0.04 & n/a & 0.08 & 1.96\\
        Linear & 32 & 0.04 & n/a & 0.08 & 2.05\\
        Linear & 64 & 0.04 & n/a & 0.08 & 2.00\\
        Linear & 128 & 0.04 & n/a & 0.08 & 2.03\\
        Linear & 256 & 0.04 & n/a & 0.08 & 1.99\\
        Linear & 512 & 0.03 & n/a & 0.07 & 2.17\\
        \hline
        Embedding & 16 & 0.01 & n/a & 0.04 & 2.76\\
        Embedding & 32 & 0.01 & n/a & 0.04 & 2.82\\
        Embedding & 64 & 0.01 & n/a & 0.04 & 2.83\\
        Embedding & 128 & 0.01 & n/a & 0.04 & 2.82\\
        Embedding & 256 & 0.01 & n/a & 0.04 & 2.80\\
        Embedding & 512 & 0.01 & n/a & 0.04 & 2.85\\
        \hline
        MHA & 16 & 0.37 & 0.39 & 0.57 & 1.54\\
        MHA & 32 & 0.36 & 0.39 & 0.58 & 1.60\\
        MHA & 64 & 0.37 & 0.39 & 0.57 & 1.54\\
        MHA & 128 & 0.37 & 0.39 & 0.57 & 1.55\\
        MHA & 256 & 0.47 & 0.47 & 0.58 & 1.23\\
        MHA & 512 & 0.83 & 0.83 & 0.83 & 1.00\\
        \hline
        RNN & 16 & 1.33 & 8.34 & 15.92 & 11.98\\
        RNN & 32 & 1.47 & 8.10 & 15.64 & 10.67\\
        RNN & 64 & 1.54 & 8.11 & 15.70 & 10.17\\
        RNN & 128 & 1.56 & 8.13 & 15.70 & 10.06\\
        RNN & 256 & 1.57 & 9.55 & 18.30 & 11.62\\
        RNN & 512 & 1.65 & 9.63 & 18.36 & 11.12\\
        \hline
        GRU & 16 & 1.49 & 22.77 & 32.66 & 21.90\\
        GRU & 32 & 1.52 & 22.52 & 32.39 & 21.30\\
        GRU & 64 & 1.59 & 22.51 & 32.41 & 20.40\\
        GRU & 128 & 1.54 & 25.43 & 36.34 & 23.53\\
        GRU & 256 & 1.66 & 25.63 & 36.23 & 21.84\\
        GRU & 512 & 1.86 & 25.90 & 36.38 & 19.51\\
        \hline
        LSTM & 16 & 1.54 & 21.16 & 29.23 & 19.00\\
        LSTM & 32 & 1.57 & 20.57 & 29.20 & 18.63\\
        LSTM & 64 & 1.38 & 22.31 & 32.74 & 23.74\\
        LSTM & 128 & 1.61 & 22.38 & 32.82 & 20.35\\
        LSTM & 256 & 1.82 & 22.37 & 32.91 & 18.12\\
        LSTM & 512 & 1.97 & 22.43 & 32.97 & 16.76\\
     \hline
\end{tabular}
\end{center}
\caption{Same as \cref{tab:runtime} but for one forward pass only.}
\label{tab:runtime_forward}
\end{table}
